A search for signatures of Europa's atmosphere and plumes in Galileo charged particle data

Remote sensing observations indicate that Europa is surrounded by a tenuous atmosphere. Furthermore, recent observations and historic data from Galileo hint at the occurrence of water vapour eruptions originating from the interior that create 200 km high plumes. Due to the lack of adequate measurements large uncertainties exist in the properties of Europa's atmosphere (e.g. loss rate and structure) and plumes (e.g. structure, source location, duration), of the latter one the existence is not even confirmed. Unexploited opportunities to constrain properties of the atmosphere or plumes remain in the in-situ data collected by the Galileo mission, the only mission that has surveyed Europa from close by. In this thesis, I investigate how to constrain the properties (density, scale height) of Europa's tenuous atmosphere and plumes, using data from the Galileo in-situ particle detector instruments (PLS, EPD). I simulate the depletion of energetic protons and oxygen ions measured during the E12 flyby. A Monte Carlo particle tracing method is used to simulate the particle trajectories and determine where they are depleted: at the surface or in the atmosphere. The simulations show that the depletions of energetic ions observed in the range 80 to 540 keV can be explained by charge exchange with neutral atmospheric particles, but not by impact on the surface alone. This suggests that an atmosphere must have been present during the E12 flyby. The simulations best represent the sublimated component of the atmosphere and favour higher surface densities than the literature, but are not sensitive to the scale height. Furthermore, an additional depletion is visible very briefly in the energetic protons with energies from 540 to 1040 keV. This feature could be consistent with localized losses from a Europa plume, although such a solution is not unique.

==> chapters/acronyms.tex <==
PWS
PLS


==> chapters/ch_introduction/ch_background.tex <==
%\chapter{Europa and its environment}
%\label{ch_background}

%In this chapter we will introduce Europa and its environment. First Europa itself, its atmosphere, neutral torus and plumes are presented (Section~\ref{s_europa_object}). Next, since plasma and energetic charged particles are key to this thesis, Europa's magnetosopheric environment and the interaction will be discussed (Section \ref{s_mag_environment}). Special emphasis is put on the interaction of plasma and energetic charged particles with Europa, which are discussed in the dedicated Section \ref{s_mag_interaction_epd_pls}.
%
%\begin{figure}[h]
%  \centering
%  \includegraphics[width=0.75\textwidth]{introduction/europa_jupiter.jpg}
%  \caption{Europa in front of Jupiter, photographed by Voyager 1 on March 3rd 1979. [NASA/JPL-Caltech/Kevin M. Gill, CC BY 2.0].}
%  \label{img_europa_jupiter}
%\end{figure}

==> chapters/ch_plume/ch_plume.tex <==
\chapter{Possible plume signatures in charged particle data during the E12 flyby}\label{ch_plume}


==> chapters/ch_search/ch_search.tex <==
\chapter{The search for plume signatures in Galileo particles and field data}\label{ch_search}




==> chapters/ch_search/s_analysis.tex <==
%\section{Processing of the PLS data}
%\label{a_pls_processing}
%
%%\subsection{Processing of the PLS data}
%In this section it is described how the PLS ion data is processed. A basic description of the instrument and its operating principles are given in Section \ref{ss_galileo}. As described previously a major challenge for processing and analysing the PLS data is the poor spatial and time coverage, resulting from the malfunction of the main antenna. An additional challenge is the noise introduced in the data by penetrating radiation. This penetrating radiation consist of highly energetic particles (such as electrons) that penetrate the shielding of the instrument and directly hit the detector, without passing through the electrostatic analyser.
%
%For the processing of the data a modified version of the CCATI software, originally developed by Markus Fr{\"a}nz, was utilized. Prior to this thesis already several fundamental steps of PLS data processing were implemented in this software, development of the software continued as part of this thesis project. 
%
%%\textcolor{red}{how to differentiate between Markus' work and mine}
%
%The raw PLS data is obtained from NASA's Planetary Data System (PDS). In this thesis we are only using the HIGH{\_}RES product. The raw data is available in units of counts per second. Besides the measurement, for every data point a time tag, the number of the respective detector, the energy bin number and the sector number are available. The sector number represents the spin angle at which the measurement was made.
%
%\subsection{Energy spectrum}
%\begin{figure}[h]
%  \centering
%  \includegraphics[width=1.0\textwidth]{method/pls_analysis.pdf}
%  \caption{Visual overview of the PLS data processing}
%  \label{img_pls_processing}
%\end{figure}
%The PLS data is processed in several steps to compensate for the poor coverage in time and energy, and remove the effect of the background noise. Here it is described how the raw data in count per second is converted into an omnidirectional energy spectrum, and converted into units of cm$^{-2}$ s$^{-1}$ sr$^{-1}$ eV$^{-1}$, referred to as differential flux or intensity. A visual overview of the different steps is provided in Figure \ref{img_pls_processing}.
%
%Per detector, for the same timetag, multiple data points with different sector numbers can be available in the raw data. To deal with this, the data is averaged over the sectors for each detector separately, this works as follows. Every single data value from a certain energy bin is averaged with the data value from the previous and next time step, corresponding to the same energy bin, but having different sector numbers.
%
%%\textcolor{red}{this is not really clear, check code, how far apart can they be?}
%
%The next issue to deal with is the sparse coverage of energy bins. After the sector averaging, a cubic spline interpolation is applied to fill in the empty energy bins. 
%
%Subsequently the noise due to penetrating radiation is removed. First the contribution of the noise is estimated based on the count rate in the four highest energy bins. The average and standard deviation are taken from the count rate values in these bins. Empty bins are neglected for this procedure. The noise is then removed by subtracting the sum of the average and the standard deviation multiplied by 0.2. This procedure of noise removal is equivalent to previous PLS studies, such as \cite{Paterson1999} and \cite{Frank1999b}.
%
%Next, averaging in time is performed together with averaging over the seven detectors. The 'box car' averaging method is used for this. This is implemented as follows, first the time frame is divided in equally sized bins, then all the values in each energy-time bin (taken from all the detectors) are summed up and finally this sum is divided by the number of values in the energy-time bin. Here we average over bins of 60 seconds in length. Figure \ref{img_pls_processing_compare} shows the data before and after processing in units of count/s. This data product can be seen for the other flybys in the figures in Section \ref{app_overview}.
%
%\begin{figure}[h]
%  \centering
%  \includegraphics[width=1.0\textwidth]{data_multi_instrument/E12_processing.pdf}
%  \caption{Top panel: unprocessed data, bottom panel: processed data. This example is the E12 flyby.}
%  \label{img_pls_processing_compare}
%\end{figure}
%
%The units of the data (prior to box car averaging) can be converted from counts/s to cm$^{-2}$ s$^{-1}$ sr$^{-1}$ eV$^{-1}$. This is done by using the calibration data provided in the PDS. Calibration data are provided as a factor that has to be multiplied with the data. This factor is referred to as 'chi-factor'. The chi-factor was obtained by the PLS team from calibration experiments in laboratory. Box car averaging is performed in the same way as described previously. The resulting data product in units of cm$^{-2}$ s$^{-1}$ sr$^{-1}$ eV$^{-1}$ can be seen in the figures in Section \ref{app_overview}. Two further data products can be derived from the differential flux: the plasma velocity magnitude and the density, these are discussed in the next section. 
%
%The PLS data collected during the close Europa flybys has generally been obtained with two different scanning modes: one low-energy mode that only scans below 15 eV and one that scans above 15 eV. Because of uncertainties in the processing of the low energy scans, we only consider data above 15 eV to be reliable.
%
%\subsection{Other data products}
%In Section \ref{app_overview} the following additional data products are also shown:
%\begin{itemize}
%\item \textbf{Density: }plasma density is calculated from the differential flux, by integrating the differential flux in every energy bin and taking the sum. This is done using Equation \ref{eq_pls_dens}, which is based on \cite{Fraenz2007}.
%\begin{equation}
%\rho = 4\pi \sum J_i \Delta E_i \frac{\sqrt{m_{factor}}}{\sqrt{E_i}}1.686e^{-8}
%\label{eq_pls_dens}
%\end{equation}
%In this Equation $J_i$ is the differential flux of the bin in cm$^{-2}$ s$^{-1}$ sr$^{-1}$ eV$^{-1}$, $\Delta E_i$ the energy width of the bin in eV, ${E_i}$ the energy of the bin in eV and $m_{factor}$ expresses the mass of the particles in amu, density $\rho$ is then in $cm^{-3}$. We use a mass factor of 18.5, this is based on Table \ref{tab_properties_magnetosphere}.
%
%%\textcolor{red}{complete}
%% plasma density is calculated from the differential flux, prior to box car averaging
%\item \textbf{Velocity magnitude: }a method is implemented to estimate the velocity magnitude of the corotational plasma. It is determined by first multiplying every energy bin with the corresponding energy bin width and converting the energy of the bin with the highest value into a velocity. The multiplication of differential flux and energy bin width scales with the count rate. This method thus looks for the bin with the highest probability of particle detections, we consider this a reliable way to estimate the velocity of the corotational plasma. Since the corotational plasma is the dominant source of plasma, the bin with the most detected particles should correspond to the corotational plasma.
%% The velocity magnitude is calculated after the box car averaging. 
%%or the purpose of this work new functions were added that
%\end{itemize}
%
%%     '/cm^3': FOR i=0,nelen-1 DO datarr[*,i]=datarr[*,i]*chi_factor[i]*denergy[i]/SQRT(energy[i])*SQRT(massfactor)*1.686e-8
%
%%We use a mass factor of ?? based on ??.
%
%%  'Density': BEGIN
%%  datout=TOTAL(datout[*,eindex],2,/nan)*4*!pi
%%  ytitle=thisvar+'!C /cm^3 R'+STRTRIM(reduc,2)
%%  yrange=[0.01,500.0]
%
%%For the purpose of this work new functions were added that:
%%- Mvel
%
%\subsection{PLS instrument pointing}
%Determining the pointing of the PLS instrument and linking observed features to a direction in physical space has been traditionally difficult. This is due to an absence of SPICE kernels and a lack of clear and consistent documentation. \cite{Bagenal2016} and supplementary material therein have documented several key points needed to understand instrument pointing and provided corrections for the documentation provided in \cite{Frank1992}. Following the suggestions of \cite{Bagenal2016} we implemented our own code to understand the looking direction of PLS. We do this by providing figures of PLS data in a non-spinning spacecraft frame, which has a constant orientation with respect to physical directions such as the corotational plasma.  This frame shares its z-axis with the spin axis of the spacecraft. We plot the data as a function of the polar angle by separating it in polar bins and azimuth bins, both in the non-spinning spacecraft frame. We determine the polar and azimuth angles as follows, using information from \cite{Bagenal2016}. For the polar angle:
%\begin{itemize}
%\item We define the polar angle of the data as the polar angle with respect to the z-axis (spin-axis) in the spacecraft frame. The polar angles of the PLS detectors in the spinning spacecraft frame are known. The number of polar bins is seven, this is because there are seven detectors, each with a different polar angle.
%\item A direction of interest (such as that of the corotational plasma) can be transformed to the spacecraft frame (available in SPICE as SC{\_}BUS = -77000), in which the polar angle of the direction can be calculated. It is then clear which detectors are best covering this polar angle.
%\end{itemize}
%For the azimuth angle:
%\begin{itemize}
%\item We define the azimuth angle as the azimuth angle in a non-rotating spacecraft frame.
%\item Since Galileo is spinning, the spin angle of each detector is continuously changing. To account for the spin, every data point has a sector number. This sector number expresses the spin angle corresponding to the measurement. The key difficulty is finding which direction sector 0 corresponds to.
%\item Sector numer 0 occurs when PLS detector 1 and 7 are in the plane containing the north pointing vector in the ECL50 reference frame (this is the vector [0,0,1] in that frame).
%\item No SPICE kernel is available for the ECL50 frame, but ECL50 north is (approximately) the same as +Z in the ECLIPB1950 reference frame, which is available in SPICE.
%\item By knowing the orientation of directions of interest (such as that of the corotational plasma) in the ECLIPB1950 frame it can be determined which sector numbers cover which directions. We divide the azimuth range in 8 parts and separate the data for each part, so that a plot can be made that shows the data in each part of the full azimuth range.
%\end{itemize}
%We have converted the following physically interesting directions in the non-spinning spacecraft frame:
%\begin{itemize}
%\item The direction of Jupiter, for this we use the IAU Europa x-axis
%\item The direction of the corotating plasma, for this we use the y-axis of the IAU Europa frame
%\item The rotation axis of Europa, which is the z-axis of the IAU Europa frame
%\item The ram direction of the spacecraft, which is the velocity of the spacecraft in the IAU frame, thus the velocity relative to Europa.
%\end{itemize}
%
%% ECL50_north
%
%% ECL50_north = np.array([0,0,1])
%% practically the same as ECLIPB1950	
%
%% ECTOR_ID	=	  0	   is	  when  PLS	   detector	 1	  and	detector   7	  are   in	   the	  plane	   containing	
%  
%% ECL-­‐50   ‘north’,   which   is   +Z   in   SPICE   frame   ECLIPB1950.	
%  


==> chapters/ch_search/s_epd_overview.tex <==
\section{EPD data overview}\label{s_epd_overview}

In this section a general description of the EPD data collected during the Europa flybys of Europa is provided.

Paranicas2000: \textcolor{red}{Unable to determine relative contribution of protons/S/O in LEMMS channels}


\subsection{Comparison of flux in different channels}

In Figure \ref{img_epd_all} the flux in, respectively, the A0\textunderscore O1, TP1\textunderscore16, TO2\textunderscore16 and TS1\textunderscore16 channel are shown for all periods when the Galileo spacecraft was within 0.5 $R_J$ of Europa's orbit. The highest flux measurements in the A0\textunderscore O1 channel corresponds to the E12 flyby.

\begin{figure}%
\centering
\subfigure[][]{%
\label{fig:ex3-a}%
\includegraphics[height=2in]{epd/a0_all_flybys.pdf}}%
\hspace{1pt}%
\subfigure[][]{%
\label{fig:ex3-b}%
\includegraphics[height=2in]{epd/tp1_all_flybys.pdf}} \\
\subfigure[][]{%
\label{fig:ex3-c}%
\includegraphics[height=2in]{epd/to2_all_flybys.pdf}}%
\hspace{1pt}%
\subfigure[][]{%
\label{fig:ex3-d}%
\includegraphics[height=2in]{epd/ts1_all_flybys.pdf}}%
\caption[A set of four subfigures.]{Flux in the A0\textunderscore O1, TP1\textunderscore16, TO2\textunderscore16 and TS1\textunderscore16 channels for all periods when the Galileo spacecraft was within 0.5 $R_J$ of Europa's orbit. Coloured points indicate close flybys, crosses indicate close flybys with hga data:
\subref{fig:ex3-a} A0\textunderscore O1 channel ;
\subref{fig:ex3-b} TP1\textunderscore16 channel;
\subref{fig:ex3-c} TO2\textunderscore16 channel; and,
\subref{fig:ex3-d} TS1\textunderscore16 channel.}%
\label{img_epd_all}%
\end{figure}

\textcolor{red}{Missing: equivalent plots with LT (Jupiter/Europa) and magnetic latitude on the x-axis}.

\subsection{Upstream-downstream wake flybys}

This section describes the flybys that passed from upstream to downstream, through the wake of Europa. These flybys are E4, E11 and E15.

\subsubsection{E4}

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{data_multi_instrument/ql_19961219_062059.pdf}
  \caption{E4 flyby data}
  \label{img_E4_all}
\end{figure}

E4 (Figure \ref{img_E4_all}) is one of the flybys that passes through the geometric wake of Europa. It moves from upstream to downstream on the Jupiter facing side of Europa. This description of the data is divided in two parts based on the geometry of the flyby. The first part concerns the time frame 06:50 - 06:55, this is the time period before Galileo enters the geometric wake and is referred to as the 'pre-geometric wake' period. The second period is from 06:55 to 07:08 and concerns the passage through Europa's geometric wake. \textcolor{red}{Refer to figure of the trajectory with time tags and indication of wake}

\textbf{Pre-geometric wake 06:50-06:55}
\begin{itemize}
\item At the beginning of the pre-geometric wake (06:50) the flux in the electron channels decreases sharply, reaching a plateau that remains approximately constant until the end of the pre-geometric wake (06:55). \textcolor{red}{I need to discuss what causes the decrease, if not the wake}
\item At the beginning of the plateau (2 minutes before the closest approach at 06:51) a strong decrease in flux in A, TP, TO and TS channels is visible. This decrease is not visible in the electron data, suggesting the difference in gyroradius is of importance to explain this feature.  \textcolor{red}{Direction of depletion still to be discussed}
\item In the middle of the plateau there is a smaller dropout in E, A, TS, TO and TP channels. \textcolor{red}{Discuss}
\item A 90-degree pitch angle depletion in the A channel \textcolor{red}{(specify which)} can be observed throughout the plateau period. Since the CA is at 688 km, the dropouts are too far from the moon to be explained by direct surface interaction. \textcolor{red}{Not only mention what happens in the A channel, but also TP,TS,TO}.
\item From PLS a decrease in corotational plasma velocity can be distinguished in the pre-geometrical wake. \textcolor{red}{link with Paterson1999 paper that discusses PLS data of this flyby}
\item Between the first depletion mentioned and the middle of the plateau the magnetic field strength decreases and reaches a minimum where the second mentioned depletion occurs. \textcolor{red}{Specify time}
\item \textcolor{red}{Discuss PWS density (increase in plasma density, seems to follow trend of electron channels)}
\end{itemize}
    
\textbf{Geometric wake 06:55-07:08}
\begin{itemize}
\item At the beginning of this period, where the plateau in the electron channels ends, a large dropout is observed in E, A, TS, TO and TP channels.
\item The flux in the electron has a generally upward trend until the end of the geometrical wake at 07:08, where the depletion ends. This implies there is no radial component in the corotational plasma.
\item Another large dropout in the middle of the geometric wake (07:00) in A, TP, TO and TS is observed. Two smaller such features can be seen at 06:58 and 07:02.  \textcolor{red}{Discuss/interpret}
\item The 90 degree pitch angle depletion in A1 continues throughout the geometrical wake and ends around 07:08.\textcolor{red}{compare with other channels}
\end{itemize}

\textcolor{red}{General note: comparison with literature, Paterson1999, Rubin2015 needed...}

\textcolor{red}{
MAG data not included yet,
- first large dropout in this region is accompanied with a short increase,
- second large dropout is accompanied with a short and sudden decrease,
- occurrence magnetic features for other dropouts are unclear}

\textcolor{red}{PWS, compare with PLS}

\subsubsection{E11}

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{data_multi_instrument/ql_19971106_200459.pdf}
  \caption{E11 flyby data}
  \label{img_E11_all}
\end{figure}

E11 (Figure \ref{img_E11_all}) is one of the flybys that passes through the geometric wake of Europa. It moves from upstream to downstream on the anti-Jovian side of Europa.
\begin{itemize}
\item Between approximately 21.45 and 21.55 a depletion of electrons can be observed. At the same time depletions in the TP channels can be distinguished, while depletion features in TS and TO channels are relatively small. This is an effect of the gyroradius and bounce period. Electrons have small radii and cannot reach the wake after having been depleted by interaction with the surface. More massive particles have larger gyroradii and can enter the wake. \textcolor{red}{link to introduction section describing the physical principles behind this}
\item The depletion feature in the A channels is centred at the 90 degree pitch angle.  \textcolor{red}{Figure needed, TS,TO,TP 90 deg pitch angle needed}.
\item From  \textcolor{red}{Figure???} it is obvious that the wake feature does not coincide with the passing through Europa's geometrical wake. The wake is shifted with  \textcolor{red}{??degree} towards Jupiter. This indicates the corotational flow has a radial component. 
\item No noticeable features are visible in the A, TP, TS and TO channels at the closest approach to Europa.
\item MAG: wake is accompanied by a feature in mag, first increase, higher frequencies and then decrease. \textcolor{red}{This wake has been described earlier by Kivelson and Volwerk, references to previous literature are needed.}
\item After the wake there is an increase in the electron flux, accompanied with a decrease in corotation flux. The feature doesn't show up in EPD ions, MAG or PLS.
\end{itemize} 

\subsubsection{E15}

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{data_multi_instrument/ql_19980531_203959.pdf}
  \caption{E15 flyby data}
  \label{img_E15_all}
\end{figure}

The E15 flyby (Figure \ref{img_E15_all}) is one of the flybys through Europa's geometrical wake. It moves from upstream to downstream on the anti-Jovian side of Europa.
\begin{itemize}
\item Between approximately 21.15 and 21.30 a depletion in electrons is visible. This depletion is accompanied with a depletion in the TP channels, but no noticeable depletion in TO or TS channels.
\item As Figure \textcolor{red}{???} shows the depletion is completely inside the geometrical wake and symmetrical with respect to the middle of the geometrical wake. It is also slightly smaller than the geometrical wake. This implies the corotational flow during this flyby has no radial component.
\item As explained in \textcolor{red}{???} the depletion features just described are typical for a wake. PLS data obtained during the wake show an increase in plasma density, that could be related to pick-up ions. \textcolor{red}{Link to Volwerk paper describing pickups in this environment} \textcolor{red}{link with earlier publications of Kivelson, magnetic feature of wake similar to that in E11}
\item At the end of the wake feature, where the flux in the electrons channels returns to the ambient level again, the electron channels follow the same trend as in the DC2 and DC3 channels. \textcolor{red}{discuss}
\item No noticeable features are visible in the A, TP, TS and TO channels at the closest approach to Europa.
\item \textcolor{red}{90 degree pitch angle depletion: possibly present from 21:14 (so several minutes before start of wake signature) until the end of the wake signature}
\end{itemize} 

\textcolor{red}{I should mention that Paranicas2000 doesn't mention E15 is actually an equatorial pass...}

\subsection{Comparing E4-E11-E15}

E11 and E15: appear broadly similar in EPD and MAG.
E4: very different from the other two in all instruments (EPD, PLS, MAG) ->
interaction is visible outside the purely wake region

\subsection{Upstream-downstream non-wake flybys}
\subsubsection{E6}

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{data_multi_instrument/ql_19970220_163459.pdf}
  \caption{E6 flyby data}
  \label{img_E6_all}
\end{figure}

E6 (Figure \ref{img_E6_all}) is one of the flybys that passes from upstream to downstream, without passing through Europa's geometrical wake. It flies by Europa on the Jupiter-facing side. No magnetic field data is available for this flyby, limiting the possibilities to compare it to others.

\begin{itemize}
\item The lower e channels are generally disturbed throughout the flyby. \textcolor{red}{What does it mean?} 
\item A peak in the lower E channels can be observed slightly before 16:50 in lower electrons, it is accompanied with a change in the plasma conditions as measured by PLS.
\item From around 4 min before CA to around 7 after CA there are dropouts in the higher A channels, TS, TO and TP, but not in E. Dropouts in A, TP, TO and TS become deeper and wider with increasing energy. The surface of Europa is within the gyroradius of at least some of the ions species. These dropouts could be related to loss because of direct interaction with the surface. \textcolor{red}{gyroradii numbers needed}
\end{itemize}

\subsubsection{E12}

E12 (Figure \ref{img_E6_all}) is one of the flybys that passes from upstream to downstream, without passing through Europa's geometrical wake. It flies by Europa on the anti-Jupiter-facing side. As discussed previously in \textcolor{red}{??} this flyby stands out because of the highest plasma density (PLS/PWS), highest magnetic field strength and largest zone in which the corotational plasma is slowed down by Europa. Noticeable features in EPD data are:
\begin{itemize}
\item A general decrease in the electron flux can be observed with respect to the closest approach.
\item A large depletion feature is observed at around 12:01 in TP, TO and TS channels. The feature is also visible in A channels, but mostly in the higher A channels. \textcolor{red}{Discuss direction.} In the electrons a dip at 12:02 can be observed. The depletion feature coincides with the highest magnetic field strength and the end of the corotation deceleration.
\item Preceding and following the large depletion feature depletions can be observed in TP between 12:01 and 12:06, in TO and TS between 12:59 and 12:09. Thus the extent of the depletions is larger in TP and TS. The depletion features become deeper with energy in TP, TO and TS. \textcolor{red}{discuss reasons and direction of features}
\item In the higher TO and TS channels larger dropout features can be observed at 11:59 and 12:09 than directly after 11:59 and directly before 12:09.
\item There is a 90 deg depletion feature in A0 and A1 channels that extends from 12:00 to 12:16. Since closest approach occurs at 12:03 this feature is clearly asymmetrical with respect to Europa. \textcolor{red}{Discuss what happens in the other channels.} The surface of Europa is not in reach of the gyroradii during part of this depletion feature. This implies a different source of losses such as charge exchange with exospheric particles could be occurring.
\end{itemize} 

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{data_multi_instrument/ql_19971216_114000.pdf}
  \caption{E12 flyby data}
  \label{img_E12_all}
\end{figure}

\subsubsection{E14}

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{data_multi_instrument/ql_19980329_130000.pdf}
  \caption{E14 flyby data}
  \label{img_E14_all}
\end{figure}

The EPD data collected during the E14 flyby (Figure \ref{img_E14_all}) does not contain any clear signatures of interaction with Europa. Between approximately 13:16 and 13:20 a dip in flux in the lower electron channels can be observed. This feature has no counterpart in the other instruments. The magnetic field strength peaks near the closest approach.

\subsubsection{E19}

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{data_multi_instrument/ql_19990201_014500.pdf}
  \caption{E19 flyby data}
  \label{img_E19_all}
\end{figure}

The EPD data collected during the E19 flyby (Figure \ref{img_E19_all}) is generally featureless. At the closest approach a depletion in TS channels and TO4 can be observed. These depletions are around the 45 degree pitch angle \textcolor{red}{figure}. The closest approach occurs at 1444 km. This is significantly larger than the gyroradii involved \textcolor{red}{numbers needed}.
The magnetic field magnitude peaks at the closest approach. \textcolor{red}{discuss}.

\subsection{Overall comparison E6-E12-E14-E19}

E6, E14 and E19 pass through similar regions as E12, but show less activity. \textcolor{red}{expand}
Is E6 a light version of E12?

\subsection{Upstream flybys - E26}

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{data_multi_instrument/ql_20000103_172000.pdf}
  \caption{E26 flyby data}
  \label{img_E26_all}
\end{figure}

The E26 flyby (Figure \ref{img_E26_all}) is the only flyby that passes through the upstream regime of Europa only.
\begin{itemize}
\item There is a sharp dip in electron flux just before the closest approach in all electron channels. \textcolor{red}{discuss, give electron gyroradius and describe if the surface can be reached or not}
\item The sharp dip in electron flux corresponds to a change in observed conditions in PLS \textcolor{red}{noise?}
\item Symmetrical with respect to the closest approach are two depletion features in the flux in the A, TS, TO and TP channels. The first one of these corresponds in time to the large dips in electrons.
\item The depletions increase in depth momentarily around 18:04. This makes the interaction region asymmetric with respect to the closest approach. After the closest approach Galileo travels in the sunward and Jupiter facing direction.
\item The depletion features near closest approach are not focused on the 90 deg pitch angle in A and TS channels. \textcolor{red}{extend to TO and TP}
\item The magnetic field increases with respect to the closest approach. Just before the closest approach coinciding with the dip in electrons and the first depletion feature is a very strong decrease in the magnetic field strength (several nT). Of the Europa flybys this feature is unique.
\item PWS reports a decrease in density with respect to the closest approach, a small increase is present at the closest approach.\textcolor{red}{figure}
\end{itemize}

\subsection{Local time}


